KP-RED: Exploiting Semantic Keypoints for Joint 3D Shape Retrieval and Deformation

In this paper, we present KP-RED, a unified KeyPoint-driven REtrieval and Deformation framework that takes object scans as input and jointly retrieves and deforms the most geometrically similar CAD models from a pre-processed database to tightly match the target. Unlike existing dense matching based methods that typically struggle with noisy partial scans, we propose to leverage category-consistent sparse keypoints to naturally handle both full and partial object scans. Specifically, we first employ a lightweight retrieval module to establish a keypoint-based embedding space, measuring the similarity among objects by dynamically aggregating deformation-aware local-global features around extracted keypoints. Objects that are close in the embedding space are considered similar in geometry. Then we introduce the neural cage-based deformation module that estimates the influence vector of each keypoint upon cage vertices inside its local support region to control the deformation of the retrieved shape. Extensive experiments on the synthetic dataset PartNet and the real-world dataset Scan2CAD demonstrate that KP-RED surpasses existing state-of-the-art approaches by a large margin. Codes and trained models are released on https://github.com/lolrudy/KP-RED.

==> Sections/Sections-backup/1-introduction-backup.tex <==
\section{Introduction}



\iffalse
1 background. has important applications in real world
2 recent progress has been made in shape understanding, but still face some problems.
3 previous methods employs XXX [list a lot of methods in a concise manner]
4 But the still fail in some cases due to several challenges.
5 To address the challenge ,we propose KP-RED
6 analyze the advantages of keypoint based method over other methods, fine with both partial and full input, semantic consistency, etc
6 to summarize, our main contributions are as follows,


\fi

Creating high-quality 3D models from object scans has received growing interest due to its wide applications in 3D scene perception~\cite{nie2020total3dunderstanding, zhang2021holistic} and artistic creation~\cite{uy2020deformation, uy2021joint}. 
Neural shape generation methods have been developed recently, but they are not good at preserving fine-grained geometric structures.~\cite{tatarchenko2019single, nie2020total3dunderstanding}
% TODO MORE?
To address this problem, \textbf{Retrieval} and \textbf{Deformation} (\textbf{R$\&$D}) methods~\cite{nan2012search,schulz2017retrieval,dahnert2019joint,wang20193dn,uy2021joint,  uy2020deformation,yifan2020neural,jiang2020shapeflow,jakab2021keypointdeformer} are proposed.
These methods leverage a 3D model database to first retrieve the most similar model and then deform it to match the target point cloud, yielding a CAD model with fine-grained structural details. 

% Previous \textbf{R$\&$D} methods mainly focus on only one of the sub-procedures: either retrieval \cite{dahnert2019joint,nan2012search} or deformation~\cite{yifan2020neural,wang20193dn,jakab2021keypointdeformer, schulz2017retrieval, uy2020deformation}. 
% Since the deformation results will influence the retrieval process, considering two stages separately leads to inferior results \cite{uy2021joint}.
% % Recent works~\cite{schulz2017retrieval, uy2020deformation} propose the deformation-aware retrieval, but their performance are limited due to their fixed and non-trainable deformation modules.
% Only a few works~\cite{uy2021joint,jiang2020shapeflow} jointly study retrieval and deformation.
% \cite{uy2021joint} designs a novel loss and training strategy to jointly optimize retrieval and deformation modules.
% However, its deformation module is based on the part annotations of the database models. 
% The part annotations are laborious to obtain and the reconstruction quality highly depends on the accuracy of the annotations.
% %Moreover, experiments show that its generalization ability on partial point cloud is limited.
% \cite{jiang2020shapeflow} adopts a flow-based deformation module to improve reconstruction quality and utilizes an auto-decoder to extract features for retrieval.
% However, the auto-decoder needs to perform time-consuming and computational-expensive online optimization during inference, which limits its use in real-world applications.
% Moreover, these methods are not robust when handling partial inputs, which are common in real-world scenario due to (self-)occlusion.
However, existing {R$\&$D} methods  typically suffer from 2 problems. 
First, most methods adopts the global feature by pooling the point features as the input of the {R$\&$D} module.
The pooling operation inevitably produces information loss, leading to relatively inferior retrieval models and coarse deformation results.
The local information should be utilized to generate finer-grained geometric structures and preserve details.
Second, partial point clouds are common in real-world scenario due to (self-)occlusion.
These methods are not robust when handling incomplete inputs since they usually treat each point equally.
However, the point distribution of partial point cloud is not uniform.
The region with higher point density should contain more useful information and contribute more to the {R$\&$D} process.
% Third, the deformation-aware retrieval is under development, which is essential since the deformation results will influence the retrieval process.


To tackle these issues, we present KP-RED, a \textbf{K}ey\textbf{P}oint-driven joint \textbf{RE}trieval and \textbf{D}eformation method.
\cite{jakab2021keypointdeformer} proposes a novel unsupervised method to deform shapes through automatically discovered 3D keypoints, which has no requirements of extra annotations and preserves fine-grained geometric structures.
Inspired by this work, we exploit the potential of semantic keypoints thoroughly and propose a keypoint-driven framework for R\&D.
We develop the keypoint grouping technique by extracting the features within each keypoint region, i.e., the neighbourhood of the keypoint.
Keypoint grouping constrains locality driven by semantic keypoints, which not only ensures semantic consistency of features extracted from each region, but also improves robustness towards partial input.
Since the unsupervised keypoints possess consistent semantic meaning in the same category, the features extracted from each keypoint region also have similar consistency.
% 1 retrieval
Based on the semantic consistency, we develop a deformation-aware retrieval module by encoding each region of the input shape into corresponding tokens.
In order to guide the network to learn deformation-aware tokens, we design an auxiliary reconstruction task which takes the deformation results into consideration.
% each token together with the target keypoints is fed into a decoder to reconstruct the corresponding deformation results of each region during training.
During inference, the token of each region is compared separately to yield precise retrieval result.
% 2 deformation
Moreover, the locality constraint enables finer-grained keypoint-driven deformation by removing redundant information and forcing network to discover the influence of each keypoint over its neighbourhood.
% 3 partial input
On the other hand, when handling partial point cloud input, there typically still remains keypoint regions which contain enough neighboring points, and the features of these regions are demonstrated to be still effective.
Therefore, we aggregate the feature and result from each region dynamically according to the point density of each region.
This dynamic region aggregation process is incorporated in both retrieval and deformation  and enhances the robustness to partial inputs.

Our main contribution are summarized as follows:
\begin{itemize}
% \item 
% We propose a novel unsupervised keypoint-driven method KP-RED, which is able to conduct retrieval and deformation for partial point cloud robustly %without extra annotations
% %capable of conducting robust joint 3D shape retrieval and deformation when facing partially-observed scanning in real world, 
% yielding state-of-the-art performance in both synthetic ShapeNet \cite{chang2015shapenet} and real Scan2CAD \cite{avetisyan2019scan2cad}.
% \item
% A keypoint grouping technique is developed to constrain locality and ensure semantic consistency of the features, which allows region-based retrieval and fine-grained deformation.
% \item
% We exploit dynamic region aggregation to handle partial point cloud in an elegant and compact manner.
\item
We present a unified network KP-RED for 3D shape generation from object scans, which learns category-consistent keypoints to jointly retrieve the most similar source shape from the pre-established database and control the shape deformation.
\item
We design a keypoint-driven local-global feature aggreation scheme to estabilsh the shape embedding space for retrieval, which performs effectively for both full and partial object scans.
\item
% KP-RED outperforms all competitors by a large margin on synthetic datasets PartNet, ComplementMe and real dataset Scannet, enabling multiple real-world applications.
We consider each keypoint's impact on shape control independently, resulting in finer-grained detail-preserving cage-based deformation.

\end{itemize}


==> Sections/Sections-backup/3-method.tex <==


\section{Method}
\subsection{Overview}
The overview of KP-RED is shown in Fig.~\ref{fig:pipeline}.
Given the target shape $S_{tgt}$, the keypoint detector predicts $N_K$ semantic keypoints $\mathbf{K}_{tgt} = \{K^{(1)}_{tgt}, K^{(2)}_{tgt}, ..., K^{(N_K)}_{tgt}\}$ and samples keypoint regions $\mathcal{R}^{(1)}_{tgt}, \mathcal{R}^{(2)}_{tgt}, ..., \mathcal{R}^{(N_K)}_{tgt}$ around each keypoint. (Sec.~\ref{sec:deform})
The retrieval module extracts deformation-resistent local-global tokens of each keypoint region $\mathcal{T}^{(1)}_{tgt}, \mathcal{T}^{(2)}_{tgt}, ..., \mathcal{T}^{(N_K)}_{tgt}$.
By comparing the tokens of the target shape and the shapes from the database region by region, the shape with the most similar tokens is selected as the source shape $S_{src}$. (Sec.~\ref{sec:retrieval})
The deformation module then estimates the keypoints of the source shape $\mathbf{K}_{src}$ by the shared keypoint predictor and associates each keypoint with its local influence region by distance-based grouping.
Finally, the deformed shape is generated by the grouped cage-based deformation via the guidance of keypoints. (Sec.~\ref{sec:deform})
When facing partial point cloud, dynamic region aggregation is employed to enhance robustness. (Sec.~\ref{sec:partial})

% \subsection{Keypoint Grouping \label{sec:group}}

% We first adopt PointNet~\cite{qi2017pointnet} to extract the per-point feature.
% Given the detected keypoints (see Sec.~\ref{sec:deform}), KP-RED then gathers the features of each keypoint region.
% The keypoint region $\mathcal{R}_i$ of keypoint $K_i$ is defined by a ball centering at $K_i$ with a fix radius $r$.
% We randomly sample $S$ points from each region and gather their features by max pooling.
% Notably, if the point number within the region is smaller than $S$, then all points in this region are sampled.

% Since the center points of the regions are keypoints with consistent semantic meaning, the features extracted in each region are also semantically consistent.
% This consistency enables region-based retrieval and yields finer-grained retrieval results (see Sec.~\ref{sec:retrieval}).
% Moreover, the keypoint grouping constrains the locality in the keypoint region, which removes redundant information and forces KP-RED to learn the keypoint's influence on its neighbourhood.
% PointNet++~\cite{qi2017pointnet++} also adopts ball query as sampling strategy.
% The main difference lies in the choice of centroids of the local regions.
% The centroids of \cite{qi2017pointnet++} are sampled via Farthest Point Sampling~(FPS), which introduces randomness and does not ensure semantic consistency.
% Also, \cite{qi2017pointnet++} samples multiple times to discover global information and does not constrain locality within region.


\subsection{Keypoint Driven Deformation \label{sec:deform}}

KP-RED learns semantic keypoints in an unsupervised manner and controls the object shape via keypoints by cage-based deformation \cite{yifan2020neural, ju2005mean} as \cite{jakab2021keypointdeformer} and extend it with distance-based grouping to boost the ability to preserve structural details.
Cage is a classical shape modeling technique~\cite{joshi2007harmonic, ju2005mean, lipman2008green} utilizing a coarse enclosing mesh to represent the outline of the shape.
The deformation of the enclosed shape can be obtained from the deformed cage mesh through interpolation by constructing mean value coordinates~\cite{ju2005mean}.

The deformation module takes the source shape $S_{src} \in \mathbb{R}^{N_P \times 3}$ and the target shape $S_{tgt} \in \mathbb{R}^{N_P \times 3}$ in the form of point cloud with $N_P$ points as input.
% Given the source shape $S_{src} \in \mathbb{R}^{N_P \times 3}$ and the target shape $S_{tgt} \in \mathbb{R}^{N_P \times 3}$, 
The keypoint predictor estimates the keypoints for both shapes $\mathbf{K}_{src}=\{ K_{src}^{(1)}, K_{src}^{(2)}, ..., K_{src}^{({N_K})}\}, \mathbf{K}_{tgt}=\{ K_{tgt}^{(1)}, K_{tgt}^{(2)}, ..., K_{tgt}^{({N_K})}\}$.

We first adopt PointNet~\cite{qi2017pointnet} to extract the per-point feature.
Given the detected keypoints, KP-RED then gathers the features of the local region around each keyopint.
The keypoint region $\mathcal{R}_i$ of keypoint $K_i$ is defined by a ball centering at $K_i$ with a fix radius $r$.
We randomly sample $N_S$ points from each region and gather their features by max pooling.
Notably, if the point number within the region is smaller than $N_S$, then all points in this region are sampled.

Then the features of each region of the source shape $g_1, g_2, ..., g_N$ are fed into the influence predictor $\Phi$ to estimate the influence vectors of each keypoint $I_1, I_2, ..., I_{N_K} \in \mathbb{R}^{N_{C} \times 3}$, where $I_i = \Phi(g_i)$ and $N_{C}$ is the number of cage vertices.
The influence vector $I_i$ describes how the displacements of keypoint $\Delta K_i$ influence the positions of cage vertices $\Delta C$ by $\Delta C = I_i \Delta K_i$.
% TODO DISTANCE-REGULARIZED
% We restrict $I_i$ to only influence at most $N_I$ nearest cage vertices of $K_i$.
% The keypoint grouping constrains the locality in the keypoint region, which removes redundant information and forces KP-RED to learn the keypoint's influence on its neighbourhood, and therefore boosting the ability to preserve structural details.
We then adopt the distance-based regularization to force $I_i$ to focus more on the local area.
We scale the influence of $I_i$ on each cage vertex according to its distance to $K^{(i)}_{src}$ hierarchically.
We sort the cage vertices by their distances to $K^{(i)}_{src}$.


We automatically obtain the source cage with cage vertices $C_{src} \in \mathbb{R}^{N_{C} \times 3}$ as \cite{jakab2021keypointdeformer, yifan2020neural} and compute the deformed cage vertices $C_{tgt}$ as follows,
\begin{equation}
    C_{tgt} = C_{src} + \sum_{i=1}^{N_K} I_i (K_{tgt}^{(i)} - K_{src}^{(i)})
\end{equation}
The deformed shape $S_{src2tgt}$ is derived from the deformed cage mesh,
\begin{equation}
    S_{src2tgt} = f_{C2S}(S_{src}, C_{src}, C_{tgt})
    \label{eq:deform}
\end{equation}
where the function $f_{C2S} : (S, C, C^*) \rightarrow S^*$ describes the cage-based deformation process~\cite{ju2005mean}, which takes the original cage $C$ and the deformed cage $C^*$ and deforms the input shape $S$ in the form of mesh or point cloud.
The deformed mesh can be obtained through $f_{C2S}$ by replacing the source point cloud with the source mesh in Eq.~\ref{eq:deform}.

We define the shape similarity loss $\mathcal{L}_{sim}$ as the Chamfer Distance between $S_{src2tgt}$ and $S_{tgt}$.
% Compared to \cite{jakab2021keypointdeformer}, we adopt keypoint grouping to ensure locality and remove redundant information, forcing the network to learn the influence of the keypoint over its neighbourhood and therefore boosting the quality of structure details.
Thanks to the strong ability of the distance-based grouping to encapsulate geometric details, we do not need the shared influence matrix across the category as well as the regularization loss on influence vectors as in \cite{jakab2021keypointdeformer}.

The keypoint regularization loss is adopted to encourage keypoints to be well-distributed by minimizing the Chamfer Distance between keypoints and $N_K$ points sampled by Farthest Point Sampling.
The final loss function of the deformation module is defined as follows,
\begin{equation}
    \mathcal{L}_{def} = \mathcal{L}_{sim} + \lambda_{kpt} \mathcal{L}_{kpt}
\end{equation}
where $\lambda_{kpt}$ is a weighting parameter.


\subsection{Deformation-Aware Region-Based Retrieval \label{sec:retrieval}}

Since the retrieval results are then refined by the deformation module, the retrieval process should take the deformation results into consideration.
In order to save computational expense and meet real-time requirement, we employ a neural encoder~\cite{xu2021you}  to encode the shape into a token which can be directly compared in the feature space for retrieval.
We design a reconstruction task and adopt a neural decoder $\Psi: (T, \mathbf{K^*}) \rightarrow S^*$ which takes the token of the source shape $T$ and the target keypoints $\mathbf{K^*}$, and reconstructs the deformation result $S^*$ of the deformation module.

We randomly select a source shape and a target shape from the training set and use the deformation module to obtain the source keypoints $\mathbf{K}_{src}$, target keypoints $\mathbf{K}_{tgt}$ and the deformed shape $S_{src2tgt}$.
Given the token of the source shape $T_{src}$ and $\mathbf{K}_{tgt}$, $\Psi$ reconstructs $S_{src2tgt}$ by
$S_{src2tgt}' = \Psi(T_{src}, \mathbf{K}_{tgt})$.
We use Chamfer Distance between $S_{src2tgt}'$ and $S_{src2tgt}$ as the loss function.
% Meanwhile, when the target keypoints are the source keypoints, the reconstruction result $S_{src}' = \Psi(T_{src}, \mathbf{K}_{src})$ should be the source shape. 
% Similarly, Chamfer Distance between $S_{src}'$ and $S_{src}$ is utilized as loss function.

If tokens of two shapes are similar, the decoder yields similar reconstruction results under the same target keypoints.
Since the decoder is trained to simulate the deformation module, the deformation results of these two shapes should also be similar.
Therefore, we obtain deformation-aware tokens by this well-designed reconstruction task.

Moreover, benefiting from the keypoint grouping, we propose a finer-grained retrieval process by encoding tokens of different keypoint regions.
Since the center points of the regions are keypoints with consistent semantic meaning, the features extracted in each region are also semantically consistent.
This consistency enables region-based retrieval and yields  precise retrieval results.

Given the token of each region from the source shape $T_{src}^{(1)}, T_{src}^{(2)}, ..., T_{src}^{(N_K)}$ and the target keypoints, $\Psi$ reconstructs each region of the deformed shape $R_{src2tgt}^{(1)}, R_{src2tgt}^{(2)}, ..., R_{src2tgt}^{(N_K)}$ correspondingly,
\begin{equation}
    {R_{src2tgt}^{(i)}}' = \Psi(T_{src}^{(i)}, \mathbf{K}_{tgt})
\end{equation}
The loss function is defined as 
\begin{equation}
    \mathcal{L}_{tgt} = \frac{1}{N_K} \sum_{i=1}^{N_K} f_{CD}(R_{src2tgt}^{(i)}, {R_{src2tgt}^{(i)}}')
\end{equation}
where $f_{CD}(\cdot, \cdot)$ is the Chamfer Distance between two shapes.


Meanwhile, $\Psi$ reconstructs the regions of the source shape $R_{src}^{(1)}, R_{src}^{(2)}, ..., R_{src}^{(N_K)}$ by the source keypoints,
\begin{equation}
    {R_{src}^{(i)}}' = \Psi(T_{src}^{(i)}, \mathbf{K}_{src})
\end{equation}
Similarly, the loss function $\mathcal{L}_{src}$ is defined by the Chamfer Distance between $R_{src}^{(i)}$ and  ${R_{src}^{(i)}}'$.
The overall loss function of  the retrieval module is 
\begin{equation}
    \mathcal{L}_{ret} = \mathcal{L}_{src} + \mathcal{L}_{tgt}
\end{equation}

During inference, the source model $\omega_{src}$ is chosen by 
% the L1 distances of the token of each region and the corresponding tokens of all shapes in the database are computed.
% We sum the distances of each region token and select the shape with the smallest sum of distances as the source shape of deformation module.
\begin{equation}
    \omega_{src} = \argmin_{\omega \in \Omega} \sum_{i=1}^{N_K} f_{L1}(T_{tgt}^{(i)}, T_{\omega}^{(i)})
\end{equation}
where $\Omega$ denotes the pre-prepared model database, $T_{\omega}^{(i)}$ is the corresponding token of model $\omega$ in the $i$th region and $f_{L1}(\cdot,\cdot)$ computes the L1 distance between the two tokens.
This strategy allows us to compare the similarity of each region respectively and obtain precise retrieval models.
Experiments prove that simply supervising on the reconstruction task yields robust tokens for retrieval.

\subsection{Handling Partial Point Cloud \label{sec:partial}}

% \subsubsection{Confidence of Keypoint Region}
% Therefore, we define the confidence of the feature and result from each region according to the point density of each region and aggregate them dynamically.
% This dynamic region aggregation process is incorporated in both retrieval and deformation  and enhances the robustness to partial inputs.

The object scannings in the real-world scenario are usually partial due to (self-) occlusion. 
Typically, the distribution of the point density is not uniform and the point density varies for each keypoint region. 
The point density inflects the robustness of the feature of the keypoint region. 
% On the other hand, when handling partial point cloud, there typically still remains keypoint regions which contain enough points, and the features of these regions will not be inflected.
Specifically, if the point density in the keypoint region is high, it is likely that the feature and the consequent output of this region is credible; if the density is low, then the result is probably erroneous.
Therefore, we utilize the point density to evaluate the confidence of the corresponding result of the region.

Since the area of each keypoint region is equal, we use the point number within each region to represent the point density.
If there are $N_R$ points in a keypoint region, then the density of the region is defined as $N_R/N_S$, where $N_S$ is the number of sampling points per region in the keypoint grouping.
The densities of all regions are denoted as $\mathbf{D} = \{D_1, D_2, ..., D_{N_K}\} \in \mathbb{R}^{N_K \times 1}$.

When facing partial input, some keypoint regions might contain no points at all.
Therefore, we add the keypoint itself to its region to avoid this situation.

\subsubsection{Retrieval}

% Given the tokens of the target shape $\mathbf{T}_{tgt}=\{T_{tgt}^{(1)}, T_{tgt}^{(2)}, ..., T_{tgt}^{(N_K)}\} \in \mathbf{R}^{N_K \times N_T}$ with $N_T$ channels,
% and the tokens of a database shape $\mathbf{T}_{db} \in \mathbf{R}^{N_K \times N_T}$, the L1 distance between them is computed as $\mathbf{E}_{L1} = | T_{tgt} - T_{db}|$.
Since the confidence of each region varies by its density, we use the density $\mathbf{D}$ to select the source model $\omega_{src}$ by 
\begin{equation}
    \omega_{src} = \argmin_{\omega \in \Omega} \sum_{i=1}^{N_K} D_i f_{L1}(T_{tgt}^{(i)}, T_{\omega}^{(i)})
\end{equation}
% $\mathbf{E}_{W} = \mathbf{D}^T \mathbf{E}_{L1} $ to evaluate the dis-similarity, where $\mathbf{D}^T$ denotes the transposition of $\mathbf{D}$.
Therefore, the region with higher density contributes more to the retrieval results, which enhances the robustness of the retrieval module in a dynamic manner.
As demonstrated in the experiments, the retrieval module trained with full shapes is robust to partial shapes.

\subsubsection{Deformation}

The source shape of the deformation module is complete since it is chosen from the database.
Also the influences of the keypoints upon the cage vertices are derived solely from the source shape.
Therefore, we only need to focus on predicting the keypoints of the partial target shape.
We adopt an additional keypoint predictor for partial shape $\Phi_{part}$ and use a trained full shape keypoint predictor $\Phi_{full}$ to guide the partial predictor in the teacher-student manner.
Since the distribution of point density is not uniform, the importance of each keypoint varies according to the density of its region.
The keypoint in a higher-density region should make more contributions on the final deformation results.
Therefore, we utilize the region density $\mathbf{D}$  to handle the difference of importance in a dynamic manner.

Given a partial shape $S_{part}$ and its corresponding full shape $S_{full}$, we obtain the keypoints of the partial shape $\mathbf{K}_{part}=\Phi_{part}(S_{part})$ and the full shape $\mathbf{K}_{full}=\Phi_{full}(S_{full})$.
The weighted keypoint loss is defined as,
\begin{equation}
    \mathcal{L}_{wkpt} = \sum_{i=1}^{N_K} D_i f_{L1}(\mathbf{K}_{full}^{(i)}, \mathbf{K}_{part}^{(i)})
\end{equation}

Meanwhile, the typical Chamfer Distance (CD) is bilateral and not suitable to evaluate shape similarity when handling partial shape.
We utilize Unilateral Chamfer Distance (UCD) of the target shape towards the deformed shape as the similarity loss, denoted as $\mathcal{L}_{usim}$.
Please refer to supplemental material for detailed information.
% The typical bilateral CD between two shapes $S_1, S_2$ is the sum of two Unilateral Chamfer Distance (UCD),
% \begin{equation}
%     \mathcal{L}_{CD}(S_1, S_2) = \mathcal{L}_{UCD}(S_1, S_2) + \mathcal{L}_{UCD}(S_2, S_1)
% \end{equation}
% where the UCD is defined as,
% \begin{equation}
%     \mathcal{L}_{UCD}(S_1, S_2) = \frac{1}{|S_1|} \sum_{x \in S_1} \min_{y \in S_2} ||x - y||_2^2
%     \label{eq:ucd}
% \end{equation}
% For each point in $S_1$, $\mathcal{L}_{UCD}(S_1, S_2)$ finds the nearest point in $S_2$, and sums the square of distance up.

% When handling partial input, the target shape $S_{tgt}$ is partial while the deformed shape $S_{def}$ is complete.
% When the deformed shape is the same as the full target shape, $\mathcal{L}_{UCD}(S_{def}, S_{tgt})$ is still large since some points in full target shape is missing in $S_{tgt}$.
% Therefore, $\mathcal{L}_{UCD}(S_{def}, S_{tgt})$  does not reflect the reconstruction quality well and we only use $\mathcal{L}_{UCD}(S_{tgt}, S_{def})$ as similarity loss, denoted as $\mathcal{L}_{usim}$.

Finally, the loss function of the deformation module when handling partial shape is defined as,
\begin{equation}
    \mathcal{L}_{pdef} = \mathcal{L}_{usim} + \lambda_{wkpt} \mathcal{L}_{wkpt}
\end{equation}
We refine the deformation module trained with full shapes and only updates the parameters of the parital shape keypoint predictor.

==> Tables/oracle.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{c|cccc}
\hline
Method & Chair          & Table           & Cabinet &Average\\
\hline
Uy \textit{et al.} &0.643  &0.564  &0.494  &0.592
 \\ 
Uy \textit{et al.} w/ IDO &0.583  &0.482  &0.494  &0.526
 \\ 
ShapeFlow  &0.167  &0.223  &0.353   &0.208  \\
Ours &\textbf{0.089}   &\textbf{0.079}  &\textbf{0.097} &\textbf{0.084} \\
\hline
\end{tabular}
\end{center}
\caption{Chamfer Distance metrics for \textbf{deformation} module using oracle retrieval. Overall best results are \textbf{in bold}.}
\label{tab:oracle}
\end{table}
